On Distributed Computation in Noisy Random Planar Networks

We consider distributed computation of functions of distributed data in random planar networks with noisy wireless links. We present a new algorithm for computation of the maximum value which is order optimal in the number of transmissions and computation time.We also adapt the histogram computation algorithm of Ying et al to make the histogram computation time optimal.

==> isit07-reviews <==
From MAILER-DAEMON Sat Mar 24 11:12:15 2007
Date: 24 Mar 2007 11:12:15 +0530
From: Mail System Internal Data <MAILER-DAEMON@bhairav.ee.iitb.ac.in>
Subject: DON'T DELETE THIS MESSAGE -- FOLDER INTERNAL DATA
X-IMAP: 1174714935 0000000000
Status: RO

This text is part of the internal format of your mail folder, and is not
a real message.  It is created automatically by the mail system software.
If deleted, important folder data will be lost, and it will be re-created
with the data reset to initial values.

From andrea@systems.stanford.edu  Fri Mar 16 06:48:42 2007
Return-Path: <andrea@systems.stanford.edu>
X-Original-To: dmanju@ee.iitb.ac.in
Delivered-To: dmanju@ee.iitb.ac.in
Received: from mailrly2.iitb.ac.in (mailrly2.iitb.ac.in [10.209.3.2])
	by bhairav.ee.iitb.ac.in (Postfix) with SMTP id 3E3386A8E
	for <dmanju@ee.iitb.ac.in>; Fri, 16 Mar 2007 06:48:42 +0530 (IST)
Received: (qmail 27863 invoked by uid 510); 16 Mar 2007 06:48:41 +0530
Received: from 72.232.50.58 by mailrly2 (envelope-from <andrea@systems.stanford.edu>, uid 502) with qmail-scanner-2.01 
 (clamdscan: 0.90.1-exp/2840. spamassassin: 3.1.7.  
 Clear:RC:0(72.232.50.58):SA:0(-4.2/4.0): Processed in 17.425232 secs); 16 Mar 2007 06:48:24 +0530
X-Spam-Checker-Version: SpamAssassin 3.1.7 (2006-10-05) on mailrly2.iitb.ac.in
X-Spam-Level: 
X-Spam-Status: No, score=-4.2 required=4.0 tests=ALL_TRUSTED,BAYES_00,SUBJ_HAS_UNIQ_ID autolearn=unavailable version=3.1.7
X-Envelope-From: andrea@systems.stanford.edu
Received: from unknown (HELO db.edas.info) (72.232.50.58)
  by mailrly2.iitb.ac.in with SMTP; 16 Mar 2007 06:48:23 +0530
Received-SPF: none (mailrly2.iitb.ac.in: domain at systems.stanford.edu does not designate permitted sender hosts)
Received: from db.edas.info (localhost.localdomain [127.0.0.1])
	by db.edas.info (8.13.1/8.13.1) with ESMTP id l2G10gH4016828;
	Thu, 15 Mar 2007 21:18:16 -0400
Received: (from root@localhost)
	by db.edas.info (8.13.1/8.13.1/Submit) id l2G0qD9C015056;
	Thu, 15 Mar 2007 20:52:13 -0400
MIME-Version: 1.0
Subject: [ISIT'07] Your paper #1569022407
Message-ID: <20070315-205213-742@edas.info>
Date: Thu, 15 Mar 2007 20:52:13 -0400
From: Andrea Goldsmith <andrea@systems.stanford.edu>
To: Yashodhan Kanoria <yashodhan@ee.iitb.ac.in>
Cc: "D. Manjunath" <dmanju@ee.iitb.ac.in>, isit07tpc-chairs@mit.edu
Content-Type: text/plain; charset="utf-8"
Content-Transfer-Encoding: 7bit
Status: R
X-Status: 
X-Keywords:                  

Dear Mr. Yashodhan Kanoria:
              
We are happy to inform you that your paper #1569022407 ('On distributed
computation in noisy random planar networks'), submitted to the IEEE
International Symposium on Information Theory 2007, has been accepted for
presentation at the symposium, and publication in the proceedings. We
received an unusually high number of paper submissions which were subjected
to a very rigorous review process. Your paper was selected for inclusion
based on its high quality and contribution. 

We encourage you to incorporate comments of the reviewers in modifying
your paper before its final submission. 

A LaTex style file is provided on the ISIT 2007  Web-site,
www.isit2007.org. For inclusion in the proceedings it is essential that the
camera-ready manuscript should have the same format as specified in this
style file. Authors are encouraged to use LaTeX and the style file to
format their camera-ready papers for the final upload.

Please note that the use of EDAS
(http://edas.info/showPaper.php?m=1569022407) is required to upload your
camera-ready manuscript. The  deadline for the receipt of the camera-ready 
manuscripts is April 20, 2007 at 11:59pm Eastern Time (New York, USA).

*****************************************************************
IMPORTANT INFORMATION FOR AUTHORS:

* Authors' registration:
In order to be included in the final program, at least one author must
register to ISIT'07 for each  accepted paper (with a maximum of two papers
registered  by  the  same  author).  The  deadline  for  early registration
is also  April 20,  2007, and  the registration  form is available  on the
ISIT'07  Web-site, www.isit2007.org.  **Accepted papers with  no registered
authors will  not be included  in the final program**. In order to link 
your registration form to a paper, please use the  following five-digit 
PAPER IDENTIFIER NUMBER:  22407.  You have to report this number in the
registration form.

* IEEE Copyright form:
A  signed IEEE  copyright  form  must be  provided  for each  accepted
paper. Papers without  copyright form **will not be  included** in the
final program.  A  pdf  version of  the  IEEE copyright  form can  be
downloaded from EDAS  (http://edas.info/showPaper.php?m=1569022407). The
copyright form must  be signed and sent by FAX to: +39-0115184666.

*****************************************************************

The reviews are attached below or can be found at
http://edas.info/showPaper.php?m=1569022407.

We look forward to seeing in Nice. 

Our Best Regards,

Andrea Goldsmith
Muriel Medard
Amin Shokrollahi
Ram Zamir

The ISIT 2007 TPC Chairs

*****************************************************************
===== Review =====

*** Importance: How important / interesting is the topic addressed in this
paper?
Average Importance (3)

*** Technical Level: Do the results seem correct (as far as you can
tell)?
Are they deep?
Technically sound (3)

*** Novelty: How novel is the paper?
Average Novelty (3)

*** Presentation: How clear is the presentation and writing of the paper?
Good (4)

*** Recommendation: Given your assessment of the paper's overall value and
assuming an expected acceptance rate around 65%, please give
your recommendation for including this paper in the ISIT'07 technical
program.
Recommend (4)

*** Strengths: What are the key strengths of this paper?


*** Weaknesses: What are the major weaknesses of this paper?


*** Comments and Recommendation: Please give the reasoning for your
overall recommendation and
any additional comments you wish to add.
This paper studies function computation in noisy random planar networks.
The authors first consider computation of the MAX function in a network
where nodes have binary data. A two-stage algorithm is proposed, where the
intra-cell computation adapts the algorithm in [5], and the inter-cell
computation adapts the spanning-tree method in [1]-[3] and the tree codes
proposed in [7]. The energy consumption of this algorithm is claimed to be
\Theta(n) under the energy model 2, and \Theta(n\log n) under the energy
model 1. The probability of error is shown to be at most \epsilon. The
authors also show that thes results can be extended to non-binary data and
block computation straightforwardly. Besides the MAX function computation,
the authors also consider the histogram computation. The problem of
histogram computation was introduced in [1], where an algorithm using
\Theta(n\log\log n) transmissions has been proposed. The authors in this
paper consider the computation time of histogram computation, which was
ignored in [1], and show that the computation time is \Theta(\sqrt{n/log
n}), which is order optimal. 

This paper demonstrates that the MAX function can be computed using order
optimal algorithm, and histogram can be obtained using an algorithm which
has the optimal time complexity. The stage-2 of the algorithm for the MAX
function divides the spanning-tree into sub-stages, and uses the tree codes
on each sub-stage to reduce the time complexity, which is quite
interesting.

Energy assumption: On page 2, the authors claimed that “results in [3]
indicate that for sufficiently large n (>=5000), it is reasonable to assume
that the transmission energy is constant and independent of n”. The
energy expenditure in [3] contains the transmission energy, receiving
energy and computation energy. The receiving and computation energy are
constant and dominate the transmission energy for large n, so the energy
expenditure in [3] is constant for large n. However, the transmission
energy is still a function of n, so the results of this paper under energy
model 2 should multiply a factor of \Theta((\sqrt{\log n/n})^\alpha) as in
[1]. 

Typos: 
(1)	On page 2, “Energy model EM_1 will refer to the case when E is is
not”.
(2)	On page 3, “From observation 2.1, [5] C_j”. 
(3)	The title of reference [3] is not complete.

===== Review =====

*** Importance: How important / interesting is the topic addressed in this
paper?
Very Important (4)

*** Technical Level: Do the results seem correct (as far as you can
tell)?
Are they deep?
Technically sound (3)

*** Novelty: How novel is the paper?
Average Novelty (3)

*** Presentation: How clear is the presentation and writing of the paper?
Average (3)

*** Recommendation: Given your assessment of the paper's overall value and
assuming an expected acceptance rate around 65%, please give
your recommendation for including this paper in the ISIT'07 technical
program.
Borderline (3)

*** Strengths: What are the key strengths of this paper?
Paper considers the question of computing symmetric function in a random
network
with minimum number of "message exchanges" in a distributed manner. The
question 
is of great interest. The solution is a straightforward mixtures of known
results.

*** Weaknesses: What are the major weaknesses of this paper?
Even though paper does take interesting results from various papers
(across disciplines), the eventual solution is somewhat straightforward.

*** Comments and Recommendation: Please give the reasoning for your
overall recommendation and
any additional comments you wish to add.
Borderline acceptance.

===== Review =====

*** Importance: How important / interesting is the topic addressed in this
paper?
Average Importance (3)

*** Technical Level: Do the results seem correct (as far as you can
tell)?
Are they deep?
Good technical level (4)

*** Novelty: How novel is the paper?
Average Novelty (3)

*** Presentation: How clear is the presentation and writing of the paper?
Good (4)

*** Recommendation: Given your assessment of the paper's overall value and
assuming an expected acceptance rate around 65%, please give
your recommendation for including this paper in the ISIT'07 technical
program.
Recommend (4)

*** Strengths: What are the key strengths of this paper?
Clear exposition

*** Weaknesses: What are the major weaknesses of this paper?
Unclear motivation for studying MAX function; insufficient explanation of
computational complexity of given algorithms; insufficient justification
for simplifying assumptions

*** Comments and Recommendation: Please give the reasoning for your
overall recommendation and
any additional comments you wish to add.
The paper presents an interesting technically sound approach to the
problem of distributed computation in noisy networks. 

It is unclear why the authors looked at the maximum function. A longer
exposition on the computational complexity aspects of the paper would have
been nice.

===== TPC Review =====



